Connectivity Damage to a Graph by the Removal of an Edge or a Vertex

The approach of quantifying the damage inflicted on a graph in Albert, Jeong and Barabsi's (AJB) report "Error and Attack Tolerance of Complex Networks" using the size of the largest connected component and the average size of the remaining components does not capture our intuitive idea of the damage to a graph caused by disconnections. We evaluate an alternative metric based on average inverse path lengths (AIPLs) that better fits our intuition that a graph can still be reasonably functional even when it is disconnected. We compare our metric with AJB's using a test set of graphs and report the differences. AJB's report should not be confused with a report by Crucitti et al. with the same name. Based on our analysis of graphs of different sizes and types, and using various numerical and statistical tools; the ratio of the average inverse path lengths of a connected graph of the same size as the sum of the size of the fragments of the disconnected graph can be used as a metric about the damage of a graph by the removal of an edge or a node. This damage is reported in the range (0,1) where 0 means that the removal had no effect on the graph's capability to perform its functions. A 1 means that the graph is totally dysfunctional. We exercise our metric on a collection of sample graphs that have been subjected to various attack profiles that focus on edge, node or degree betweenness values. We believe that this metric can be used to quantify the damage done to the graph by an attacker, and that it can be used in evaluating the positive effect of adding additional edges to an existing graph.

==> Equations/adjacencyMatrix.tex <==
 A_{ij} = \left\{ \begin{array}{ll}
                     1 & \mbox{if there is an edge between vertices $i$ and $j$} \\
		     0 & \mbox{otherwise.}
                    \end{array}
	    \right.


==> Equations/aipl.tex <==
\item Average inverse path length (AIPL) \cite{holme2002attack}.\\
 The average of the inverse  of all shortest paths 
between all nodes $u$ and $v$.  AIPL is also known as average
inverse shortest path (AISP) \cite{beygelzimer2005improving} and average inverse shortest path length (AISPL) \cite{venuturumilli2006obtaining}.
\MyEquationLabeled{averageDistanceInverse}{equ:02c}
If a path does not exist between nodes $u$ and $v$   then by definition the path's length is infinite $\infty$.


==> Equations/allI2J.tex <==
i \rightarrow j:\forall _{i,j} \in V


==> Equations/apl.tex <==
\item Average path length (APL)\cite{brinkmeier211}.\\
 The average of all shortest path lengths  between nodes $u$ and $v$. 
The  lower an APL, the fewer edges on average there are between nodes.
 \MyEquationLabeled{averageDistance}{equ:01c}


==> Equations/aplConstrained.tex <==
\item Constrained average path length (CAPL).\\
 The average of all shortest path lengths  between nodes $u$ and $v$, 
given that there is a path between  $u$ and $v$.
The  lower an CAPL, the fewer edges on average there are between nodes.
 \MyEquationLabeled{averageDistanceConnected}{equ:01d}


==> Equations/averageDegreeLHS.tex <==
\ensuremath {\left \langle \MyEquationInline{edgesLHS} \right \rangle }


==> Equations/averageDegreeRandom.tex <==
\MyEquationInline{averageDegreeLHS} = \frac {2m}{n} = p(n-1) \approx pn


==> Equations/averageDistance.tex <==
\MyEquationInline{averageDistanceLHS} = \frac {1}{n(n-1)} \sum_{u \neq v \in V} d(u,v)


==> Equations/averageDistanceConnected.tex <==
\MyEquationInline{averageDistanceLHS} =  \frac {1}{n(n-1)} \sum_{\stackrel{u \neq v \in V}{0 < d(u,v) < \infty}} d(u,v)


==> Equations/averageDistanceInverse.tex <==
\MyEquationInline{averageDistanceLHSinverse} =  \frac{1}{n(n-1)} \sum_{u \neq v \in V}  \frac{1}{d(u,v)}


==> Equations/averageDistanceLHS.tex <==
\ensuremath{L(G)}


==> Equations/averageDistanceLHSinverse.tex <==
\ensuremath{L(G)^{-1}}


==> Equations/averageDistanceLattice.tex <==
\MyEquationInline{averageDistanceLHS} \sim \frac {n}{2k} \gg 1


==> Equations/averageDistanceSocial.tex <==
\MyEquationInline{averageDistanceLHS} = \propto \log N


==> Equations/averagePathLength.tex <==
\MyEquationInline{averageDistanceLHS} =\frac{1}{n*(n-1)}*\sum_{i,j}^{n}d(v_{i},v_{j})


==> Equations/averagePathLengthRandom.tex <==
\MyEquationInline{averageDistanceLHS} \sim \frac{\text{ln}(n)}{\text{ln}(k)}


==> Equations/averagePathLengthSmallWorld.tex <==
\MyEquationInline{averageDistanceLHS} \sim \frac {n}{2k}


==> Equations/betweennessEdge.tex <==
\MyEquationInline{betweennessEdgeLHS} = \sum_{s \neq t \in V} \frac{\sigma _{st}(e)}{\sigma _{st}}


==> Equations/betweennessEdgeLHS.tex <==
\ensuremath{c_{B}(e)}


==> Equations/betweennessGlobalEdge.tex <==
\MyEquationInline{betweennessGlobalEdgeLHS} = max(\MyEquationInline{betweennessEdgeLHS} | e \in E)


==> Equations/betweennessGlobalEdgeLHS.tex <==
\ensuremath{c_{B}(E)}


==> Equations/betweennessGlobalVertex.tex <==
\MyEquationInline{betweennessGlobalVertexLHS} = max(\MyEquationInline{betweennessVertexLHS} | v \in V)


==> Equations/betweennessGlobalVertexLHS.tex <==
\ensuremath{c_{B}(V)}


==> Equations/betweennessVertex.tex <==
\MyEquationInline{betweennessVertexLHS} = \sum_{s \neq v \neq t \in V} \frac{\sigma _{st}(v)}{\sigma _{st}}


==> Equations/betweennessVertex1.tex <==
c_{B}(v) = |\sigma _{st}(v) : s \neq v \neq t \in V|


==> Equations/betweennessVertexLHS.tex <==
\ensuremath{c_{B}(v)}


==> Equations/center.tex <==
\MyEquationInline{centerLHS}=\{u \in V:r(G) = e(u)\}


==> Equations/centerLHS.tex <==
\ensuremath{C(G)}


==> Equations/centralityDegreeLHS.tex <==
\ensuremath{c_{D}(v)}


==> Equations/closeness.tex <==
\MyEquationInline{closenessLHS} = \sum_{v \in V}d(u,v)


==> Equations/closenessLHS.tex <==
\ensuremath{c_{C}(u)}


==> Equations/closenessNormalized.tex <==
\MyEquationInline{closenessLHS} = \frac {n - 1}{   \sum_{u \neq v \in V}d(u,v)}


==> Equations/clusteringAverage.tex <==
\MyEquationInline{clusteringAverageLHS} = \frac{1}{n}\sum_{i}\frac{Number \quad  Of  \quad Triangles
 \quad Connected  \quad To  \quad Vertex  \quad i}{Number  \quad Of  \quad
Triples  \quad Centered  \quad At  \quad Vertex \quad  i}


==> Equations/clusteringAverage02.tex <==
\MyEquationInline{clusteringAverageLHS} = \frac {\MyEquationInline{neighborhoodEdges}}{ \binom{\MyEquationInline{edgesLHS}_{v}}{2}}


==> Equations/clusteringAverageLHS.tex <==
\ensuremath{\MyEquationInline{clusteringCoefficientGlobalLHS}_{Average Local}}


==> Equations/clusteringAverageTriple.tex <==
\MyEquationInline{clusteringAverageTripleLHS} = \frac{1}{\sum_{i, C_{i} \ne 0}}\sum_{i}\frac{{Number
 \quad Of  \quad  Triangles  \quad Connected  \quad To  \quad Vertex  \quad
i}}{{Number  \quad Of  \quad Triples  \quad Centered  \quad At  \quad Vertrx \quad  i}}


==> Equations/clusteringAverageTripleLHS.tex <==
\ensuremath{\MyEquationInline{clusteringCoefficientGlobalLHS}_{AverageTriples}}


==> Equations/clusteringCoefficient.tex <==
\MyEquationInline{clusteringCoefficientLocalLHS} = \frac {2 * \lambda (v) } { d(v)^{2} - d(v)}


==> Equations/clusteringCoefficient02.tex <==
\MyEquationInline{clusteringCoefficientLocalLHS} = 
\frac {\MyEquationInline{triangleLocalLHS}}{\MyEquationInline{tripleLocalLHS}}


==> Equations/clusteringCoefficientGlobalAverageLHS.tex <==
\ensuremath{\MyEquationInline{clusteringCoefficientGlobalLHS}_{Average}}


==> Equations/clusteringCoefficientGlobalLHS.tex <==
\ensuremath{C(G)}


==> Equations/clusteringCoefficientGlobalLatticeLHS.tex <==
\ensuremath{\MyEquationInline{clusteringCoefficientGlobalLHS}_{Lattice}}


==> Equations/clusteringCoefficientLocalLHS.tex <==
\ensuremath{c(v)}


==> Equations/clusteringCoefficientRandom.tex <==
\MyEquationInline{clusteringCoefficientGlobalLHS}  \sim \frac{k}{n}


==> Equations/clusteringCoefficientSmallWorld.tex <==
\MyEquationInline{clusteringCoefficientGlobalLHS} \sim \frac{3}{4}


==> Equations/clusteringGlobal.tex <==
\MyEquationInline{clusteringCoefficientGlobalAverageLHS} = \frac{3 * \Sigma Number\quad Of \quad Triangles \quad In \quad The
\quad Graph}{Number \quad Of \quad Connected \quad Triples}


==> Equations/clusteringLattice.tex <==
\MyEquationInline{clusteringCoefficientGlobalLatticeLHS}= \frac{(3k-3)}{2(2k-1)}


==> Equations/clusteringLatticeRewiredLHS.tex <==
\ensuremath{\MyEquationInline{clusteringCoefficientGlobalLHS}_{LatticeRewired}}


==> Equations/clusteringRewired-02.tex <==
\MyEquationInline{clusteringLatticeRewiredLHS} = \frac{(3k-3)}{(4k-2)}*(1-p)^{3}


==> Equations/clusteringRewired.tex <==
\MyEquationInline{clusteringRewiredLHS} = C(C^{k}_{n})(1 - \frac{p}{2k})


==> Equations/clusteringRewiredLHS.tex <==
\ensuremath{\MyEquationInline{clusteringCoefficientGlobalLHS}_{Rewired}}


==> Equations/damage-01.tex <==
\delta = 1 - \frac{max_{i}\mid C_{i} \mid}{\mid C_{0}\mid}

==> Equations/damage-02.tex <==
\ensuremath{\MyEquationInline{damageLHS} = 1 - \frac{L(G_{fragmented})^{-1}}{L(G_{unfragmented})^{-1}}}


==> Equations/damage-03.tex <==
\ensuremath{\MyEquationInline{damageLHS} = \mid \mathclose 1 - \frac{L(G_{fragmented})^{-1}}{L(G_{unfragmented})^{-1}} \mathclose \mid}


==> Equations/damage.tex <==
\MyEquationInline{damageLHS} = 1 - \frac{\operatorname*{max} (\mid C_{i} \mid): \forall C \in \{C\}}{n}


==> Equations/damageLHS.tex <==
\ensuremath{Damage(G)}


==> Equations/degree.tex <==
\ensuremath{d(v) = \MyEquationInline{edgesLHS}}


==> Equations/degreeConnectivity.tex <==
\delta (G)


==> Equations/degreeDirectedInDegree.tex <==
c_{iD}(v) = d^{-}(v)


==> Equations/degreeDirectedOutDegree.tex <==
c_{oD}(v) = d^{+}(v)


==> Equations/degreeMaximalGlobal.tex <==
\ensuremath{\Delta(G)}


==> Equations/degreeMinimalGlobal.tex <==
\ensuremath{\delta(G)}

==> Equations/degreeUndirectedDegree.tex <==
c_{D}(v) = d(v)


==> Equations/density1.tex <==
\MyEquationInline{densityLHS} = \frac{m}{n}


==> Equations/density2.tex <==
\MyEquationInline{densityLHS} = (\frac{n^{2}}{2m}-1)(1-\frac{1}{n}) 


==> Equations/density3.tex <==
\MyEquationInline{densityLHS} = \frac{m}{\binom{n}{2}}


==> Equations/densityLHS.tex <==
\ensuremath{\rho(G)}


==> Equations/diameter.tex <==
\MyEquationInline{diameterLHS} = max\{\MyEquationInline{distance}\}


==> Equations/diameterLHS.tex <==
\ensuremath{D(G)}


==> Equations/distance.tex <==
d(u,v):u,v \in V


==> Equations/distanceEdge.tex <==
d(u,v)= \mathclose \mid E(P) \mathclose \mid, E(P) = \{u_0u_1,u_1u_2,\ldots,v_{-1}v_0\}


==> Equations/distanceVertex.tex <==
d(u,v)= \mathclose \mid V(P) \mathclose \mid, V(P) = \{u_0,u_1,\ldots,v_{-1},v_0\}


==> Equations/eccentricity.tex <==
\MyEquationInline{eccentricityLocalLHS}=max\{d(u,v):v\in V\}


==> Equations/eccentricityGlobal.tex <==
\MyEquationInline{eccentricityGlobalLHS}=max\{\MyEquationInline{eccentricityLocalLHS}:u\in V\}


==> Equations/eccentricityGlobalLHS.tex <==
\ensuremath{\MyEquationInline{eccentricitySymbolLHS}(G)}


==> Equations/eccentricityLHS.tex <==
\ensuremath{\epsilon}


==> Equations/eccentricityLocalLHS.tex <==
\ensuremath{\MyEquationInline{eccentricitySymbolLHS}(u)}


==> Equations/eccentricitySymbolLHS.tex <==
\ensuremath{\epsilon}


==> Equations/edgeConnectivity.tex <==
\lambda (G)


==> Equations/edgeLHS.tex <==
\ensuremath{E}

==> Equations/edgesLHS.tex <==
\ensuremath{k}

==> Equations/eigenMatrix.tex <==
 A x = \lambda x


==> Equations/exponentialLaw.tex <==
 \MyEquationInline{probKLHS}=\lambda e^{-\lambda k}


==> Equations/exponentialLaw2.tex <==
 \log \MyEquationInline{probKLHS} = -\lambda k + log \lambda


==> Equations/fScore.tex <==
\MyEquationInline{fScoreLHS} = \frac{2 * \textrm{precision} * \textrm{recall}}{\textrm{precision} + \textrm{recall}}


==> Equations/fScoreBeta.tex <==
%\MyEquationInline{fScoreBetaLHS} = (1+ \beta^{2})\frac{x_{1}x_{2}}{\beta^{2}x_{1}+x_{2}}
\MyEquationInline{fScoreBetaLHS} = (1+ \beta^{2})\frac{\textrm{precision} * \textrm{recall}}{\beta^{2}\textrm{precision} + \textrm{recall}}


==> Equations/fScoreBetaLHS.tex <==
\ensuremath {F_{\beta}}


==> Equations/fScoreLHS.tex <==
\ensuremath {F_{score}}


==> Equations/geometricMean.tex <==
\MyEquationInline{geometricMeanLHS} = \sqrt[n]{x_{1}x_{2}...x_{n}}


==> Equations/geometricMeanLHS.tex <==
\ensuremath {G}


==> Equations/globalEfficiency.tex <==
 \MyEquationInline{globalEfficiencyLHS} = \frac{1}{n(n+1)} \sum_{i \neq j \in V} \frac{1}{d_{ij}}


==> Equations/globalEfficiency2.tex <==
\MyEquationInline{globalEfficiencyLHS} = \frac{1}{n(n-1)} \sum_{i \neq j \in V} \frac{1}{d_{ij}}


==> Equations/globalEfficiencyLHS.tex <==
\ensuremath {E(G)}


==> Equations/globalRobustness.tex <==
 \MyEquationInline{globalRobustnessLHS} = \frac{E_{t}}{E}


==> Equations/globalRobustnessLHS.tex <==
\ensuremath{R(G)}


==> Equations/graph.tex <==
\MyEquationInline{graphLHS}

==> Equations/graphLHS.tex <==
\ensuremath{G(\MyEquationInline{vertexLHS.tex},\MyEquationInline{edgeLHS.tex})}


==> Equations/graphSize.tex <==
S = \left\{
\begin{array}{l l}
  (2*PL, D(G)) & \text{if Power Law} \\
   \MyEquationInline{averageDegreeLHS}^{PL} & \text{if Random} \\
  (2*PL, D(G))  & \text{if Watts---Strogatz small-world} \\
\end{array} \right.


==> Equations/harmonicMean2.tex <==
\MyEquationInline{harmonicMeanLHS} = \frac{2x_{1}x_{2}}{x_{1}+x_{2}}


==> Equations/harmonicMeanGeneral.tex <==
\MyEquationInline{harmonicMeanLHS} = \frac {n} {\frac{1}{x_{1}} + \frac{1}{x_{2}} + ... + \frac{1}{x_{n}}}


==> Equations/harmonicMeanLHS.tex <==
\ensuremath{H}


==> Equations/importantNeighbors.tex <==
 x_{i}=\frac{1}{\lambda}\sum_{j=1}^{n}A_{ij}x_{j}


==> Equations/latoraDamageWorst.tex <==
\ensuremath{\MyEquationInline{latoraDamageWorstLHS}=\Phi[D(S,d^{*})]}


==> Equations/latoraDamageWorstLHS.tex <==
\ensuremath{W[S,D]}


==> Equations/latoraPerformance.tex <==
\ensuremath{\MyEquationInline{latoraPerformanceLHS}>0}


==> Equations/latoraPerformanceLHS.tex <==
\ensuremath{\Phi[S]}


==> Equations/latoraVulnerability.tex <==
\MyEquationInline{latoraVulnerabilityLHS} = \frac{\MyEquationInline{latoraPerformanceLHS} - \MyEquationInline{latoraDamageWorstLHS}}{\MyEquationInline{latoraPerformanceLHS}}


==> Equations/latoraVulnerabilityLHS.tex <==
\ensuremath{V[S,D]}


==> Equations/meanDegree.tex <==
c_{D}(G)=\frac{1}{n}\sum_{i=1}^{n}c_{d}(v_{i})


==> Equations/neighborhoodEdges.tex <==
\ensuremath{\mid \Gamma_{v} \mid _{\mathcal{E}}}


==> Equations/neighborhoodVertices.tex <==
\ensuremath{\mid \Gamma_{v} \mid _{\mathcal{V}}}


==> Equations/notallI2J.tex <==
i \nrightarrow j:\exists _{i,j} \in V

==> Equations/numberVertices.tex <==
\ensuremath{n}

==> Equations/numberVerticesLHS.tex <==
\ensuremath{n}

==> Equations/pa.tex <==
 \MyEquationInline{probKLHS} = ck^{-\delta} |  \MyEquationInline{subjectTo1}


==> Equations/pathLHS.tex <==
\ensuremath{\delta _{st}}

==> Equations/powerLaw.tex <==
 \MyEquationInline{probKLHS} = Ck^{-\alpha}


==> Equations/powerLaw2.tex <==
\log  \MyEquationInline{probKLHS} = -\alpha \log k + \log C


==> Equations/preferentialAttachment.tex <==
 \MyEquationInline{probKLHS} = ck^{-\delta} | \MyEquationInline{subjectTo1}


==> Equations/probKLHS.tex <==
\ensuremath {p(k)}


==> Equations/quadraticMean.tex <==
\MyEquationInline{quadraticMeanLHS} = \sqrt{\frac{x_{1}^{2} + x_{2}^{2} +...+ x_{n}^{2}}{n}}


==> Equations/quadraticMeanLHS.tex <==
\ensuremath{Q_{rms}}


==> Equations/radius.tex <==
\MyEquationInline{radiusLHS}=min\{\epsilon (u):u \in V\}


==> Equations/radiusLHS.tex <==
\ensuremath{r(G)}


==> Equations/randomGnmLHS.tex <==
\ensuremath{G_{n,m}}


==> Equations/randomGnpLHS.tex <==
\ensuremath{G_{n,p}}


==> Equations/rewireNguyen.tex <==
p=d(u,v)^{-r}

==> Equations/shortestPathEdge.tex <==
\MyEquationInline{pathLHS}(e) = \frac{ \sigma _{st}(e)} {\sigma_{st}}


==> Equations/shortestPathVertex.tex <==
\MyEquationInline{pathLHS}(v) = \frac{ \sigma _{st}(v)} {\sigma_{st}}


==> Equations/structural.tex <==
 S_{c}(G)=\{u \in V : \forall v \in V \: c(u) \geq c(v)\} 


==> Equations/subjectTo1.tex <==
\delta > 0, c > 0


==> Equations/test.tex <==
a = \input{/home/chuck/LEdProjects/Styles/Equations/vertexConnectivity.tex}


==> Equations/triangle.tex <==
\triangle = \{V_{\triangle},E_{\triangle}\}


==> Equations/triangleGlobal.tex <==
\MyEquationInline{triangleGlobalLHS} = 
\mathclose \mid \{ \MyEquationInline{triangleLocalLHS} \in V_{\triangle}\}\mathclose \mid


==> Equations/triangleGlobalLHS.tex <==
\ensuremath{\lambda(G)}


==> Equations/triangleLocal.tex <==
\MyEquationInline{triangleLocalLHS} = \mathclose \mid \{ \triangle \mid v \in V_{\triangle}\}\mathclose \mid


==> Equations/triangleLocalLHS.tex <==
\ensuremath{\lambda(v)}


==> Equations/tripleGlobal.tex <==
\MyEquationInline{tripleGlobalLHS} = \sum _{v \in V} \MyEquationInline{tripleLocalLHS}


==> Equations/tripleGlobalLHS.tex <==
\ensuremath{\tau(G)}


==> Equations/tripleLocal.tex <==
\MyEquationInline{tripleLocalLHS} = \frac {d(v)^{2} - d(v)}{2}


==> Equations/tripleLocalLHS.tex <==
\ensuremath{\tau(v)}


==> Equations/vertexConnectivity.tex <==
\kappa (G)


==> Equations/vertexLHS.tex <==
\ensuremath{V}

==> Equations/vulnerability.tex <==
\MyEquationInline{vulnerabilityLHS} = \mbox{exp} \{ \frac{\sigma}{n} + n - \mathclose \mid E \mathclose \mid - 2 + \frac{2}{n} \}


==> Equations/vulnerabilityDegreeStdDev.tex <==
\MyEquationInline{vulnerabilityDegreeStdDevLHS} = \sqrt{\frac{1}{n}  \sum_{i=1}^{n} (k_{i} - \frac {2\mathclose \mid E \mathclose \mid}{n})^{2}}


==> Equations/vulnerabilityDegreeStdDevLHS.tex <==
\ensuremath {\sigma}


==> Equations/vulnerabilityLHS.tex <==
\ensuremath {v^{**}(G)}


==> Makefile <==
#SRC=secondThoughts
#SRC=thirdThoughts
#SRC=fourthThoughts
SRC=final
#SRC=temp
#LATEX=pdflatex
LATEX=latex
BIBTEX=bibtex

all:clean report

report:
	$(LATEX) $(SRC).tex
	$(BIBTEX)  $(SRC)
	$(LATEX)  $(SRC).tex
	$(LATEX)  $(SRC).tex
	dvipdfm $(SRC)

clean:
	for i in aux dvi log lot toc bbl blg;\
	do \
		rm -f $(SRC).$$i ;\
	done

